Diffuse Ionized Gas inside the dwarf irregular galaxy NGC 6822

We have studied the differences between the diffuse ionized gas (DIG) and the HII regions along a slit position in the local dwarf irregular galaxy NGC 6822. The slit position passes through the two most prominent HII regions: Hubble V and Hubble X. Important differences have been found in the excitation, ionization, and [NII]6584/Ha and [SII]6717/Ha line ratios between the DIG and the HII locations. Moreover, the values of all the line ratios are not similar to those in the DIG locations of spiral galaxies but are very similar to the values in other irregular galaxies, such as IC 10. We also determined the rate of recombination using the HeI5875 line. Finally, we obtained a picture of the ionization sources of the DIG. We consider that the leakage of photons from the HII regions might explain most of the line ratios, except [NII]/Ha, which might be explained by turbulence.

==> table1.tex <==
\begin{table*}
\scriptsize
\caption[]{ Total values of the line ratios  from the integrated spectra. Column 
1 lists the line ratios studied, while the values (extinction-corrected) for 
these ratios for the five different regions considered (from west to east) 
are shown in columns 2, 3, 4, 5 and 6.  The value of the [OII]/H$\beta$ ratio has
to be taken with care because of the extinction correction problems.(see text)} 
\vspace{0.05cm}
\begin{center}
\begin{tabular}{c c c c c  c}
\hline
{Ratio }   & {DIG W} & {Hubble V}  & {DIG C} & {Hubble X} & {DIG E}  \\ 
\hline 

$\lbrack$OII$\rbrack$$\lambda$3726+2739\AA/H$\beta$ & 5.041$\pm$0.3 & 0.485$\pm$0.02 & 3.078$\pm$0.2    & 0.859$\pm$0.04 & 2.89$\pm$0.1\\
$\lbrack$OIII$\rbrack$$\lambda$5007\AA/H$\beta$ & 1.33$\pm$0.07 & 5.246$\pm$0.3 & 1.17$\pm$0.06 & 4.161$\pm$0.2 & 2.332$\pm$0.1 \\
HeI $\lambda$5875\AA/H$\alpha$ & 0.07$\pm$0.03 & 0.036$\pm$0.003  & 0.06$\pm$0.03  & 0.040$\pm$0.003   & 0.06$\pm$0.03 \\
$\lbrack$NII$\rbrack$$\lambda$6583\AA/H$\alpha$ & 0.124$\pm$0.008 & 0.019$\pm$0.001 & 0.094$\pm$0.005 & 0.029$\pm$0.001   & 0.109$\pm$0.009  \\
$\lbrack$SII$\rbrack$$\lambda$6717\AA/H$\alpha$ & 0.122$\pm$0.006 & 0.025$\pm$0.001 & 0.119$\pm$0.006 & 0.039$\pm$0.002 & 0.112$\pm$0.006  \\
$\lbrack$OIII$\rbrack$$\lambda$5007\AA/$\lbrack$OII$\rbrack$$\lambda$3726+3729\AA & 0.263$\pm$0.02 & 10.82$\pm$0.5 & 0.382$\pm$0.02 & 4.844$\pm$0.2 & 0.807$\pm$0.4 \\
$\lbrack$SII$\rbrack$$\lambda$6717\AA/$\lbrack$SII$\rbrack$$\lambda$6731\AA & 1.62$\pm$0.09 & 1.320$\pm$0.07 & 1.392$\pm$0.07 & 1.409$\pm$0.07   & 1.829$\pm$0.09 \\ 
$\lbrack$NII$\rbrack$$\lambda$6584\AA/$\lbrack$SII$\rbrack$$\lambda$6717\AA & 1.016$\pm$0.1 & 0.76$\pm$0.05 & 0.79$\pm$0.06 & 0.74$\pm$0.05  & 0.97$\pm$0.09\\
\hline
C$_{\beta}$ & 2.33$\pm$0.01  &  -   & 1.45$\pm$0.01 &  -  & 0.708$\pm$0.001  \\
Te DIG (N) & 9228 K  &   -    & 8578  K  &   -   & 9936  K \\
Te DIG (O) & 10202 K &   -    & 9261 K   &   -   & 9698 K \\
S/N (H$\alpha$) & 8 & 23 & 9 & 21& 6 \\
\hline
\end{tabular}
\end{center}
\end{table*}


